How can LLMs Support Policy Researchers? Evaluating an LLM-Assisted Workflow for Large-Scale Unstructured Data

Policy researchers need scalable ways to surface public views, yet they often rely on interviews, listening sessions, and surveys-analyzed thematically-that are slow, expensive, and limited in scale and diversity. LLMs offer new possibilities for thematic analysis of unstructured text, yet we know little about how LLM-assisted workflows perform for policy research. Building on a workflow for LLM-assisted thematic analysis of online forums, we conduct a study with 11 policy researchers, who use an early prototype and see it as a quick, rough-and-ready input to their research. We then extend and scale the workflow to analyze millions of Reddit posts and 1,058 chatbot-led interview transcripts on a policy-relevant topic, treating these sources as rich and scalable data for policy discourse. We compare the synthesized themes to those from authoritative policy reports, identify points of alignment and divergence, and discuss what this implies for policy researchers adopting LLM-assisted workflows.

==> Sections/quote_table_label5.tex <==
\section{Themes in Online Forum Data that Do not Fall in Pre-defined Theme Groups}
\label{appendix:reddit_label_5}
\begin{longtable}{|p{2.5cm}|p{5cm}|p{6.5cm}|p{0.8cm}|}
\hline
\textbf{Theme Title} & \textbf{Theme Description} & \textbf{Quote} & \textbf{Ratio} \\
\hline
\endfirsthead

\hline
\textbf{Theme Title} & \textbf{Theme Description} & \textbf{Quote} & \textbf{Ratio} \\
\hline
\endhead

AI Tools and Automation & Exploration of AI tools and their role in automating processes and enhancing productivity & \tquote{I'm curious how AI tools might streamline this process. What are your thoughts on using AI-powered knowledge management systems to help organize and optimize all this content creation? Could it potentially improve productivity or free up time from constantly being online?} & 16.4\% \\
\hline
AI Content Quality and Ethics & Discussions on the quality, effectiveness, and ethical implications of AI-generated content & \tquote{But this guys point about AI being used by malicious actors to blur the lines [further] between reality and propagandic fantasy did make me stop and think for a bit.} & 13.7\% \\
\hline
AI in Education & Exploration of AI's role in transforming educational practices, learning tools, and academic methodologies. & \tquote{Yeah there is going to be no incentive for a lot of people to learn a lot of things. Which on some level is okay if it's not run completely by for profit companies or government.} & 9.4\% \\
\hline
AI Hype and Skepticism & Debates on the sustainability of AI trends and their real-world impact on society. & \tquote{AI \& ML is a road to broken dreams, the hype exists to milk dumb investment funds don’t get pulled down yourself. FAANG had stupid levels of hype, eventually their salaries \& promises came crashing down too. Hype surrounds unsustainable ideas.} & 5.8\% \\
\hline
Outsourcing and Global Competition & Concerns about outsourcing jobs, its financial effects, and competition from international workers. & \tquote{In the future I doubt it'll be outsourced to other countries it'll probably outsourced AI when they get that perfected. It's all about the profitability and the cheapest labor that they can get.} & 5.4\% \\
\hline
Economic Pressures and Challenges & Concerns about wage stagnation, rising costs, and economic pressures affecting various industries. & \tquote{I'm starting to think we might be forced into a revolution - if enough people can't afford rent and go broke with their backs up against the wall - well it won't be good. The cost of living is too high and you can only push so many people over the edge until it's too many and they start fighting back.} & 4.5\% \\
\hline
AI Accessibility and Affordability & Concerns regarding the cost and access to AI technologies, impacting various users and industries. & \tquote{In the medium-term, only people with access to the compute power will be empowered by AI. So many people are going to be left in the dust like farmers in Eritrea, migrants in Nicaragua, etc. etc. It will also increase the power gap between oppressors and oppressed groups like the Rohingya or Uyghur.} & 3.9\% \\
\hline
Investment Opportunities in AI & Exploration of investment strategies and opportunities related to AI technologies and sectors. & \tquote{Bank of America put out a piece saying that they expect software companies to increase AI investment significantly. They said that currently, software companies are spending around 4\% of their revenue on AI investment.} & 2.1\% \\
\hline
AI Integration and Implementation Challenges & Discussions on the difficulties and costs associated with integrating AI into products and services. & \tquote{I have a product where we are working to integrate AI into it and it performs great 95\% of the time. But that 5\% is BAD, really bad, to the point where we had to scale back use cases because the risk wasn’t worth it.} & 1.8\% \\
\hline
\caption{Themes in Online Forum Data that Do not Fall in Pre-defined Theme Groups}
\Description{The table shows online forum themes that do not fit into pre-defined groups. Themes include AI tools and automation (16.4\%), AI content quality and ethics (13.7\%), AI in education (9.4\%), AI hype and skepticism (5.8\%), outsourcing and global competition (5.4\%), economic pressures and challenges (4.5\%), AI accessibility and affordability (3.9\%), investment opportunities in AI (2.1\%), and AI integration and implementation challenges (1.8\%). Each theme has a description and a sample quote.
}
\label{tab:quotes_label_5}
\end{longtable}


